A Multi-Channel Next POI Recommendation Framework with Multi-Granularity Check-in Signals

Current study on next POI recommendation mainly explores user sequential transitions with the fine-grained individual-user POI check-in trajectories only, which suffers from the severe check-in data sparsity issue. In fact, coarse-grained signals (i.e., region- and global-level check-ins) in such sparse check-ins would also benefit to augment user preference learning. Specifically, our data analysis unveils that user movement exhibits noticeable patterns w.r.t. the regions of visited POIs. Meanwhile, the global all-user check-ins can help reflect sequential regularities shared by the crowd. We are, therefore, inspired to propose the MCMG: a Multi-Channel next POI recommendation framework with Multi-Granularity signals categorized from two orthogonal perspectives, i.e., fine-coarse grained check-ins at either POI/region level or local/global level. Being equipped with three modules (i.e., global user behavior encoder, local multi-channel encoder, and region-aware weighting strategy), MCMG is capable of capturing both fine- and coarse-grained sequential regularities as well as exploring the dynamic impact of multi-channel by differentiating the region check-in patterns. Extensive experiments on four real-world datasets show that our MCMG significantly outperforms state-of-the-art next POI recommendation approaches.

==> table/ablation_study.tex <==
\begin{table}[t]
	\centering
	\small
	\caption{Performance comparison for different combination strategy of MTL across four datasets w.r.t HR@10 and NDCG@10. \textcolor{red}{radar chart}
	}\label{tab:variants}
	\vspace{-0.15in}
	\addtolength{\tabcolsep}{-3pt}
	\begin{tabular}{l|c|c|c|c|c|c|c|c} 
	\specialrule{.15em}{.05em}{.05em}
% 		\specialrule{.05em}{.05em}{.05em}
% 		\specialrule{.05em}{.05em}{.05em}
		& \multicolumn{2}{c|}{CAL}
		& \multicolumn{2}{c|}{PHO}
		& \multicolumn{2}{c|}{SIN}
		& \multicolumn{2}{c}{NY}
		\\ \cline{2-9}
		& HR  & NDCG  & HR & NDCG & HR  & NDCG & HR  & NDCG \\ 
		\specialrule{.05em}{.05em}{.05em}
		group attention& 0.51  & 0.36 & 0.38  & 0.24  & 0.32  & 0.19& 0.25  & 0.19 \\
		overall attention & 0.50 & 0.34 & 0.36 & 0.23 & 0.30 & 0.18& 0.24 & 0.18 \\
		average pooling&	0.51&	0.32&	0.19&	0.10&	0.31 &	0.18 & 0.20 & 0.12  \\
		concatenate&	0.47 &	0.31&	0.12&	0.05&	0.30&	0.16& 0.18 & 0.10 \\
		\specialrule{.15em}{.05em}{.05em}
	\end{tabular}
	\label{table:variation}
	\vspace{-0.14in}
\end{table}

==> table/info_granularity.tex <==
\begin{table}[t]
\footnotesize
  \caption{Multi-aspect granularity information.
  }\label{tab:multi-granularities}
 \vspace{-0.1in}
  \addtolength{\tabcolsep}{-3pt}
  \begin{tabular}{l|cc}
    \specialrule{.15em}{.15em}{.15em}
    & {fine-grained information} & {coarse-grained information}\\
    \specialrule{.1em}{.1em}{.1em}
    geographical aspect & POI & region \\
    user-behavioral aspect & local (the current sequence) & global (all users' sequences)\\
  \specialrule{.15em}{.15em}{.15em}
\end{tabular}
\vspace{-0.2in}
\end{table}
